Deep Features for Contactless Fingerprint Presentation Attack Detection: Can They Be Generalized?

The rapid evolution of high-end smartphones with advanced high-resolution cameras has resulted in contactless capture of fingerprint biometrics that are more reliable and suitable for verification. Similar to other biometric systems, contactless fingerprint-verification systems are vulnerable to presentation attacks. In this paper, we present a comparative study on the generalizability of seven different pre-trained Convolutional Neural Networks (CNN) and a Vision Transformer (ViT) to reliably detect presentation attacks. Extensive experiments were carried out on publicly available smartphone-based presentation attack datasets using four different Presentation Attack Instruments (PAI). The detection performance of the eighth deep feature technique was evaluated using the leave-one-out protocol to benchmark the generalization performance for unseen PAI. The obtained results indicated the best generalization performance with the ResNet50 CNN.

==> TAbles.tex <==
%%%
\begin{table*}[htp]
\centering
\caption{Quantitative performance of the deep features for contactless fingerprint PAD}
\label{tab:PAD-table}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{}
>{\columncolor[HTML]{CBCEFB}}l lllll
>{\columncolor[HTML]{C0C0C0}}l llll@{}}
\cellcolor[HTML]{CBCEFB} &
   &
   &
  \multicolumn{3}{l}{BPCER @ APCER =} &
  \cellcolor[HTML]{C0C0C0} &
   &
   &
  \multicolumn{2}{l}{BPCER @ APCER =} \\
\cellcolor[HTML]{CBCEFB} &
  \multirow{-2}{*}{PAD Algorithms} &
  \multirow{-2}{*}{D-EER} &
  5\% &
  \multicolumn{2}{l}{10\%} &
  \cellcolor[HTML]{C0C0C0} &
  \multirow{-2}{*}{PAD Algorithms} &
  \multirow{-2}{*}{D-EER} &
  5 &
  10 \\
\cellcolor[HTML]{CBCEFB} &
  AlexNet &
  6.91 &
  \multicolumn{2}{l}{11.67} &
  3.78 &
  \cellcolor[HTML]{C0C0C0} &
  AlexNet &
  25.43 &
  61.94 &
  47.98 \\
\cellcolor[HTML]{CBCEFB} &
  GoogleNet &
  11.54 &
  \multicolumn{2}{l}{22.24} &
  13.47 &
  \cellcolor[HTML]{C0C0C0} &
  GoogleNet &
  23.63 &
  59.28 &
  43.86 \\
\cellcolor[HTML]{CBCEFB} &
  DenseNet201 &
  6.97 &
  \multicolumn{2}{l}{10.22} &
  4.43 &
  \cellcolor[HTML]{C0C0C0} &
  DenseNet201 &
  23.19 &
  63.18 &
  50.20 \\
\cellcolor[HTML]{CBCEFB} &
  ResNet50 &
  6.65 &
  \multicolumn{2}{l}{8.28} &
  3.50 &
  \cellcolor[HTML]{C0C0C0} &
  ResNet50 &
  14.58 &
  30.22 &
  20.85 \\
\cellcolor[HTML]{CBCEFB} &
  EfficientNet-B0 &
  7.21 &
  \multicolumn{2}{l}{11.15} &
  4.47 &
  \cellcolor[HTML]{C0C0C0} &
  EfficientNet-B0 &
  14.58 &
  34.05 &
  21.47 \\
\cellcolor[HTML]{CBCEFB} &
  NasNet &
  13.30 &
  \multicolumn{2}{l}{29.62} &
  17.73 &
  \cellcolor[HTML]{C0C0C0} &
  NasNet &
  30.16 &
  83.59 &
  69.01 \\
\cellcolor[HTML]{CBCEFB} &
  MobileNet-V2 &
  12.00 &
  \multicolumn{2}{l}{29.10} &
  15.14 &
  \cellcolor[HTML]{C0C0C0} &
  MobileNet-V2 &
  16.22 &
  49.40 &
  28.00 \\
\multirow{-10}{*}{\cellcolor[HTML]{CBCEFB}Case-1} &
  Vision Transformer &
  6.71 &
  \multicolumn{2}{l}{8.17} &
  3.74 &
  \multirow{-10}{*}{\cellcolor[HTML]{C0C0C0}Case-2} &
  Vision Transformer &
  50.00 &
  100.00 &
  100.00 \\
\cellcolor[HTML]{ECF4FF} &
  AlexNet &
  50.00 &
  \multicolumn{2}{l}{97.03} &
  93.99 &
  \cellcolor[HTML]{FFCCC9} &
  AlexNet &
  10.30 &
  18.84 &
  10.31 \\
\cellcolor[HTML]{ECF4FF} &
  GoogleNet &
  50.00 &
  \multicolumn{2}{l}{96.93} &
  93.01 &
  \cellcolor[HTML]{FFCCC9} &
  GoogleNet &
  4.43 &
  4.29 &
  1.88 \\
\cellcolor[HTML]{ECF4FF} &
  DenseNet201 &
  48.42 &
  \multicolumn{2}{l}{96.01} &
  91.94 &
  \cellcolor[HTML]{FFCCC9} &
  DenseNet201 &
  4.40 &
  3.98 &
  1.47 \\
\cellcolor[HTML]{ECF4FF} &
  ResNet50 &
  7.58 &
  \multicolumn{2}{l}{11.56} &
  5.49 &
  \cellcolor[HTML]{FFCCC9} &
  ResNet50 &
  2.94 &
  0.26 &
  0.05 \\
\cellcolor[HTML]{ECF4FF} &
  EfficientNet-B0 &
  25.58 &
  \multicolumn{2}{l}{72.78} &
  55.06 &
  \cellcolor[HTML]{FFCCC9} &
  EfficientNet-B0 &
  3.30 &
  1.10 &
  2.51 \\
\cellcolor[HTML]{ECF4FF} &
  NasNet &
  4.81 &
  \multicolumn{2}{l}{4.66} &
  1.75 &
  \cellcolor[HTML]{FFCCC9} &
  NasNet &
  8.55 &
  13.24 &
  6.54 \\
\cellcolor[HTML]{ECF4FF} &
  MobileNet-V2 &
  50.00 &
  \multicolumn{2}{l}{98.80} &
  96.51 &
  \cellcolor[HTML]{FFCCC9} &
  MobileNet-V2 &
  6.6 &
  7.85 &
  4.08 \\
\multirow{-8}{*}{\cellcolor[HTML]{ECF4FF}Case-3} &
  Vision Transformer &
  23.65 &
  \multicolumn{2}{l}{100.00} &
  100.00 &
  \multirow{-8}{*}{\cellcolor[HTML]{FFCCC9}Case-4} &
  Vision Transformer &
  2.57 &
  0.99 &
  0.31
\end{tabular}%
}
\end{table*}
